Tate classes and endoscopy for $\operatorname{GSp}_4$ over totally real fields

The theory of endoscopy predicts the existence of large families of Tate classes on certain products of Shimura varieties, and it is natural to ask in what cases one can construct algebraic cycles giving rise to these Tate classes. This paper takes up the case of Tate classes arising from the Yoshida lift: these are Tate cycles in middle degree on the Shimura variety for the group $\operatorname{Res}_{F/\mathbb Q} (\operatorname{GL}_2 \times \operatorname{GSp}_4)$, where $F$ is a totally real field. A special case is the family of Tate classes which reflect the appearance of two-dimensional Galois representations in the middle cohomology of both a modular curve and a Siegel modular threefold. We show that a natural algebraic cycle generates exactly the Tate classes which are associated to \emph{generic} members of the endoscopic $L$-packets on $\operatorname{GSp}_{4,F}$. In the non-generic case, we give an alternate construction, which shows that the predicted Tate classes arise from Hodge cycles.

==> theta.tex <==

 \section{Theta lifts from $\GL_2$ to $\GSO_4$}\label{sec: small lifting}
 %IN this section we need to flip $\xphi $ and $\widehat\xphi $! Exhalation point
 \subsection{Notations}
 In this subsection we consider the standard two-dimensional $F$-symplectic space $$W = \langle e_1\rangle\oplus \langle e_2\rangle$$ and the four-dimensional orthogonal $F$-space $V$ of $2\times 2$ matrices. The pairing on $V $ is defined by 
 \begin{equation}
    \langle w_1, w_2\rangle=\tr (w_1\overline w_2),
 \end{equation}
  for the standard involution on $W$ characterized by $w + \overline w = \tr(w)$.
  We will use the coordinates $$\underline x = \begin{pmatrix} x & y \\ z & w\end{pmatrix}$$ on $V$, and the complete polarization
 $ V = V_1\oplus V_2$ where \begin{equation}\label{eq:isotropic of V}
   V_1 =   \begin{pmatrix}
        x & y\\0 & 0
      \end{pmatrix},\;\; V_2 =\begin{pmatrix}0 & 0\\z & w\end{pmatrix}.
  \end{equation}\subsubsection{}
  Denote by $$\mathbf p_Z: \GL_2\times \GL_2 \to \mathrm{GO}(V)$$ the map defined by setting $$(g_1,g_2) \underline x = g_1 \underline x\overline g_2,\;\;\; \underline x\in V.$$
  Then the kernel of $\mathbf p_Z$ is the antidiagonally embedded $\mathbb G_m$, and $\mathbf p_Z$ is a surjection onto the connected orthogonal similitude group $\GSO(V)$ (the group denoted $M$ in the introduction).
  Notice that $\nu(\mathbf p_Z(g_1, g_2)) = \det(g_1)\det(g_2)$. 
  %We denote by $\mathbf P_Z: GL_2\times GL_2 \to GSO(V)$ the canonical projection.
  We will denote automorphic representations of $\GSO(V)(\A_F)$ by $\pi_1 \boxtimes \pi_2,$ where $\pi_1$ and $\pi_2$ have the same central character; likewise if $f_1,f_2$ are automorphic functions on $\GL_2(\A_F)$ with the same central character, then $f_1\otimes f_2$ denotes the automorphic function on $\GSO(V)(\A_F)$ defined by $f_1\otimes f_2 (\boldsymbol p_Z (g_1, g_2)) = f_1 (g_1) f_2 (g_2) $.
\subsubsection{}

  
 Equip $W\otimes V$ with coordinates by:
 \begin{equation}
     (x_1,y_1,z_1,w_1,x_2,y_2,z_2,w_2) \longleftrightarrow e_1\otimes \begin{pmatrix} x_1 & y_1 \\ z_1 & w_1 \end{pmatrix} + e_2 \otimes \begin{pmatrix} x_2 & y_2 \\ z_2 & w_2 \end{pmatrix}.
 \end{equation}
 We have two different complete polarizations on $W\otimes V$: 
 \begin{equation}
     W\otimes V = \langle e_1\rangle \otimes V \oplus \langle e_2\rangle \otimes V = W\otimes V_1\oplus W\otimes V_2.
 \end{equation}
 When there is no risk of confusion, we identify $e_2\otimes V $ with $V$ and give it coordinates $(x,y,z,w)$ rather than $(x_2,y_2,z_2,w_2)$.
  We consider the two models on $\mathcal S_\bullet (\langle e_2\rangle\otimes V) $ and on $\mathcal S_\bullet (W\otimes V_2) $. 
  %We shall also abbreviate by $c\mapsto h_c$ the section of $\det: GL_2 \to \mathbb G_m$ defined by $h_c = \begin{pmatrix} 1 & 0 \\ 0 & c\end{pmatrix}.$
 
  \subsection{Lifts of cuspidal representations}
  Let $\pi $ be a cuspidal automorphic representation of $\GL_2 (\A_F) $. It is well-known that the theta lift $\Theta(\pi)\subset \mathcal A_0(\GSO(V)(\A_F))$ is isomorphic to the automorphic representation $\pi\boxtimes\pi$ of $\GSO(V)$. 
  We will require the following calculation later on.
  \begin{lemma}\label{Lemma: Fourier coefficient of cuspidal left}
  Let $\xphi =\otimes_v\xphi\in\mathcal S_\A (\langle e_2\rangle\otimes W) $
  and $f =\otimes_vf_v\in\pi $ be factorizable vectors, and choose a factorization $$W_{\psi,f}(h) = \prod_v W_{f,v}(h_v),\;\; h = (h_v)\in \GL_2(\A_F)$$ of the global Whittaker function of $f$ (so that $W_f(h_v)(1) = 1$ for almost all $v$). Then the Whittaker coefficient of $\theta_\xphi (f) $ along the standard unipotent subgroup $N\times N\subset\boldsymbol p_Z (\GL_2\times \GL_2) $ is given by:
  $$\theta_{\xphi} (f) (g)_{N\times N,\psi ^ {-1}\times\psi ^ {-1}} =\prod_v\left(\integral_{\mathrm{SL}_2 (F_v)} W_{f,v} (h_vh_{c_v})\omega (h_vh_{c_v}, g)\widehat\xphi (1, 0, 0, -1)\d h_v\right),\;\; c = (c_v) =\det(g).$$
  %Here, if $f_v $ and $\xphi_v$ are  spherical and $W_{f,v} (1) = 1, $
  %then $$g_v\mapsto \integral_{SL_2 (F_v)} W_{f, v}(hh_c) \omega(hh_c,g)\widehat\xphi_v(-1,0,0,1) \d h$$ 
  \end{lemma}
  \begin{proof}
 We compute in two steps. First, for $(h,g)\in R_0(\A_F)$,
 \begin{align*}
     \theta (h,g;\xphi)_{N\times 1,\psi^{-1}\times 1}& = \integral_{[N]}\sum_{x\in W\otimes V_2}\omega(h,ng) \widehat\xphi (x)\psi (n)\d n\\
     & =\integral_{[\mathbb G_a]}\sum_{(z_1, w_1, z_2, w_2)}\psi (a (w_2z_1 - z_2w_1))\omega(h,g)\widehat\xphi (z_1, w_1, z_2, w_2)\psi (a)\d a\\
     &=  \sum_{\substack{(z_1, w_1, z_2, w_2)\\z_1w_2 - w_1z_2 = 1}}\omega(h,g)\widehat \xphi (x) \\
   &= \sum_{\gamma\in \SL_2(F)} \omega(\gamma h, g)\widehat \xphi(1,0,0,-1).
 \end{align*}
 Here $\d n$ is the Haar measure on $N$ such that $[N]$ has volume 1. 
 Now, using the identity $$\omega (n h, g)\widehat\xphi (1, 0, 0, -1)=\omega (h, \boldsymbol p_Z(1,n) g)\widehat\xphi (1, 0, 0, -1),\;\; (g, h)\in R_0,\;n\in N (\A), $$
 we obtain:
 \begin{align*}
     \theta_\xphi (f) (g)_{N\times N,\psi ^ {-1}\times\psi ^ {-1}} &=\integral_{[N]}\integral_{[\SL_2]} \theta (hh_c, \boldsymbol p_Z(1,n)g;\xphi)_{N\times 1,\psi ^ {-1}\times 1}\psi (n) f(hh_c)\d h\d n\\
     & =\integral_{[N]}\integral_{\SL_2(\A)}\omega (hh_c, \boldsymbol p_Z(1,n) g)\widehat\xphi(1,0,0,-1)\psi (n) f (hh_c)\d h\d n\\
     & =\integral_{[N]}\integral_{\SL_2(\A)}\omega ( hh_c, g)\widehat\xphi (1, 0, 0, -1)\psi (n) f (n^{-1}hh_c)\d n\d h\\
     &=\integral_{\SL_2 (\A)}\omega (hh_c,g)\widehat\xphi(1,0,0,-1)W_{\psi, f} (hh_c)\d h,
 \end{align*}
 which gives the lemma.
  \end{proof}

 \input{siegel weil}

\subsubsection{}\label{Subsubsection: Schwartz function convention}
To describe explicit Schwartz functions for this similitude theta lift, we will use the following convention. Fix a basis $\set{e_1,e_2,e_3,e_4}$ for $W $ with respect to which the symplectic pairing has the matrix:
 $$\begin{pmatrix}
       0 & 1 & 0 & 0\\
       -1 & 0 & 0 & 0\\
       0 & 0 & 0 & 1\\
       0 & 0 & -1 & 0
 \end{pmatrix}. $$
We choose the complete polarization $$W = W_1\oplus W_2 = \langle e_1,e_3\rangle \oplus\langle e_2,e_4\rangle. $$
Then the Weil representation for $\GSp_4\times V_B$ is realized on $$\mathcal S_{\A_F} (\langle e_2, e_4\rangle\otimes V_B). $$
Given two Schwartz functions $\xphi,\xphi' \in \mathcal S_{\A_F}(V_B),$ we
write $$\xphi\otimes\xphi'\in\mathcal S_{\A_F}(\langle e_2, e_4\rangle\otimes V_B)$$ for the Schwartz function determined by $\xphi\otimes\xphi' (e_2\otimes x + e_4\otimes x') =\xphi (x)\xphi' (x') $.
A similar convention applies for local Schwartz functions. Note that $\mathcal S_{F_v} (\langle e_2, e_4\rangle\otimes V_B) $
is spanned by functions of the form $\xphi\otimes\xphi' $ if $v$ is non-archimedean.

